Automorphisms of twisted Chevalley groups of type ${}^2E_6$ over local rings

We classify abstract automorphisms of the elementary and full twisted Chevalley groups of type ${}^2E_6$ over commutative local rings with involution and $2$ invertible, for both isogeny types. Every automorphism is standard, with no invertibility assumption on $3$. In the adjoint case, it has a unique expression as a composition of conjugation by an element of the full twisted group and a ring automorphism commuting with the involution. For the simply connected form, the full group equals its elementary subgroup, and the factors are strictly inner, diagonal, and ring automorphisms. The main step replaces a linear change of basis by a group element. Invariant alternating tensors determine the transported Chevalley bracket. We correct this bracket over a faithfully flat local extension and descend the resulting conjugating element by uniqueness. Root-subgroup relations then recover the coefficient automorphism.

==> twisted_e6_verification/manuscript_crosswalk.tex <==
\section*{Computational verification}

The computational parts of the proof are the complete short-root
normalization in Lemma~\ref{lemma:full-short-root-normalization},
the invariant-tensor calculation in
Lemma~\ref{lemma:invariant-alternating-tensors}, and the two
root-recognition calculations in Lemma~\ref{lemma:long-root-rigidity}.
The archive \path{twisted_e6_verification.zip} contains their source
code, exact systems, model matrices, selected rows and columns, and
certificate minors. The accompanying \path{verification_report.pdf}
and \path{verification_results.json} give the corresponding
human-readable and machine-readable summaries.

The three calculations are in
\path{sections/section4_complete_short_root/},
\path{sections/section5_invariant_tensors/}, and
\path{sections/section6_parameter_rigidity/}, respectively.
After installing the requirements listed in the archive, the command
\texttt{python run\_all.py} verifies the stored certificates and
regenerates all systems in a temporary copy, comparing the results
with the delivered data. All proof calculations are exact over
$\mathbb Z[1/2]$; the unit-minor and model-vector arguments in the
text justify arbitrary base change. The long-root relation $3u=0$
is retained until bracket preservation gives $u=0$.

Lemma~\ref{lemma:bracket-stabilizer-tangent} has a direct proof in the
text. The additional computation in
\path{sections/section5_bracket_stabilizer/} is a consistency check,
not a prerequisite for that proof. The archive also checks the
Chevalley sign conventions and the standard Weyl words.

